Class Impression for Data-free Incremental Learning

Standard deep learning-based classification approaches require collecting all samples from all classes in advance and are trained offline. This paradigm may not be practical in real-world clinical applications, where new classes are incrementally introduced through the addition of new data. Class incremental learning is a strategy allowing learning from such data. However, a major challenge is catastrophic forgetting, i.e., performance degradation on previous classes when adapting a trained model to new data. Prior methodologies to alleviate this challenge save a portion of training data require perpetual storage of such data that may introduce privacy issues. Here, we propose a novel data-free class incremental learning framework that first synthesizes data from the model trained on previous classes to generate a \ours. Subsequently, it updates the model by combining the synthesized data with new class data. Furthermore, we incorporate a cosine normalized Cross-entropy loss to mitigate the adverse effects of the imbalance, a margin loss to increase separation among previous classes and new ones, and an intra-domain contrastive loss to generalize the model trained on the synthesized data to real data. We compare our proposed framework with state-of-the-art methods in class incremental learning, where we demonstrate improvement in accuracy for the classification of 11,062 echocardiography cine series of patients.

==> trash/ethical-statements.tex <==
% \section{Compliance with Ethical Standards}
% % This is a numerical simulation study for which no ethical approval was required.
% The research work is related to human studies. The HIV and Bipolar datasets employed in this study are owned by a third-party organization, where informed consent was obtained for all subjects. The data processed is anonymous with no personally identifiable information. All studies are conducted according to the Good Clinical Practice guidelines and U.S. 21 CFR Part 50 (Protection of Human Subjects), and under the approval of Institutional Review Boards. 

% % \section{Acknowledgements}
% % No funding was received for conducting this study. The authors have no relevant financial or non-financial interests to disclose.


==> trash/experiments.tex <==
\section{Experiments}

\subsection{Datasets and Experimental Settings}
We use \hejie{three} real-world datasets from \cite{Ma:2017gl} to evaluate our framework. 
\begin{itemize}
    \item \noindent \textbf{Human Immunodeficiency Virus Infection (HIV)} is collected from functional magnetic resonance imaging (fMRI), including 35 samples from positive patients and 35 from negative healthy controls. Each graph contains 90 nodes (ROIs) and the edge weights corresponding to the adjacency matrix are calculated as the pairwise correlations between brain regions.
    \item \noindent \textbf{Bipolar Disorder (BP)} is also collected from fMRI modality, consisting of 52 bipolar subjects and 45 healthy controls with matched age and gender. It stimulates 82 brain regions, according to Freesurfer-generated cortical/subcortical gray matter regions. Functional brain networks are derived using pairwise BOLD signal correlations.
    \hejie{\item \noindent \textbf{(PPMI)} is xxxx.}
\end{itemize}

% \noindent \textbf{Node features construction.}
% \label{sec:predict_node}
% The lack of predictive original ROI features limits the power of GNNs \cite{cui2021features}. To this end, we construct multiple node features based on connections, one-hot identities as well as local statistical measures such as degree profiles (LDP) \cite{Cai:2018te}. 
% Specifically, in connection-based method, each feature \(\bm{x}_i\) of node $v_i$ is computed as $\bm{W}_i$, where \(\bm{W} \in \mathbb{R}^{m \times m}\) is the adjacency matrix of the graph. 
% Other common artificial node features such as binning degree \cite{cui2021features} and node2vec \cite{DBLP:conf/kdd/GroverL16} are also experimented as alternatives. 

\noindent \textbf{Hyper-parameter setting.}
% The proposed model is implemented using PyTorch \cite{DBLP:conf/nips/PaszkeGMLBCKLGA19} and PyTorch Geometric \cite{DBLP:journals/corr/abs-1903-02428}. 
We  use  the Adam  optimizer \cite{DBLP:journals/corr/KingmaB14} with the initial learning rate of 0.001 and a weight decay of 0.00001. The backbone model is trained for 100 epochs with hidden dimension setting to 64. \hejie{All the hyper-parameters are selected automatically with the open source AutoML toolkit NNI\footnote{https://github.com/microsoft/nni}. Besides, multiple constructed node features are tested including one-hot, binning degree\cite{cui2021features}, node2vec \cite{DBLP:conf/kdd/GroverL16}, and edge-connection, where each feature \(\bm{x}_i\) of node $v_i$ is computed the $i$th row in the graph adjacency matrix \(\bm{W} \in \mathbb{R}^{m \times m}\). To indicate the robustness of each model, all the reported results are the average performance of ten-fold cross validation conducted 
on different train/test splits}.


\subsection{Interpretability Analysis}
\label{sec:vis}
% \begin{figure}[t]
% 	\centering
% 	\subfloat[HIV]{
% 		\includegraphics[width=0.7\linewidth]{figures/hiv_vis.pdf}
% 		\label{fig:hiv_vis}
% 	}\\
% 	\vspace{-10pt}
% 	\subfloat[BP]{
% 		\includegraphics[width=0.7\linewidth]{figures/bp_vis.pdf}
% 		\label{fig:bp_vis}
% 	}
% 	\caption{Comparison of explanation graph connectomes in brain networks of a healthy control and a patient on HIV and BP datasets. The colors of neural systems are described as: {\color{sred} VN}, {\color{sgolden} AN}, {\color{sgreen} BLN}, {\color{sblue} DMN}, {\color{spurple} SMN}, {\color{spink} SN}, {\color{sorange} MN}, {\color{slightgreen} CCN}, respectively.}
% 	\label{fig:vis}
% \end{figure}

\begin{figure}[t]
% \vspace{-3pt}
\centering
    \begin{minipage}{.42\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{figures/hiv_vis_oneline.pdf}
      (a) HIV
    %   \caption{(a) HIV}
      \label{fig:hiv_vis}
    \end{minipage}%
    \begin{minipage}{.42\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{figures/bp_vis_oneline.pdf}
      (b) BP
    %   \caption{(b) BP}
      \label{fig:bp_vis}
    \end{minipage}
\caption{\label{fig:vis} Comparison of explanation graph connectomes in brain networks of a healthy control and a patient on HIV and BP datasets. The colors of neural systems are described as: {\color{sred} VN}, {\color{sgolden} AN}, {\color{sgreen} BLN}, {\color{sblue} DMN}, {\color{spurple} SMN}, {\color{spink} SN}, {\color{sorange} MN}, {\color{slightgreen} CCN}, respectively.}
\end{figure}

\textbf{\hejie{Interpretation of important connectomes}.}
To qualitatively examine the effectiveness of the globally shared mask $\bm{M}$, \hejie{we follow a similar strategy as the post processings in GNNExplainer \cite{ying2019gnnexplainer}, where \hejie{an explanation subgraph $G^{\prime}_s$ is obtained by taking the top 100 weighted edges from the masked $G^{\prime}$ and all other low-weight edges are removed.}} 
\hejie{As an illustration, we show the comparison of connectomes for healthy control and patient groups on HIV and BP datasets in Figure \ref{fig:vis}}, where edges within the same systems are colored according to the color of nodes it links, while edges across systems are colored gray. The size of an edge is decided by its weight in the explanation graph. 
% Regarding the experimented results, we have the following observations.

It can be seen that connectome patterns differ within certain neural systems between the healthy control and patient subject, which could provide potential value for clinical diagnosis. For example, in the HIV dataset, the explanation subgraph of patients excludes many interactions within the Default Mode Network system (DMN), which is colored {\color{sblue} blue}. The connections between superior frontal gyrus (nodes 3, 4) and orbital part (nodes 5, 6, 9, 10) are two examples\footnote{See \cite{chen2021decreased} for ROI names and respective node indices.}. Also, interactions within the Visual Network (VN, colored {\color{sred} red}) system of patients are significantly less than that of healthy controls. For example, connections between cuneus (nodes 45, 46) and lingual gyrus (nodes 47, 48), and those between occipital gyrus (nodes 51, 52, 53, 54) and fusiform gyrus (nodes 55, 56) are  missing. 
These patterns are consistent with the findings in \cite{herting2015default, flannery2021hiv} that alterations in within- and between-network DMN and VN connectivity may relate to known cognitive and visual processing difficulties in HIV. % HIV-infected individuals 

For the BP dataset, compared with tight interactions within the Bilateral Limbic Network (BLN, colored {\color{sgreen} green}) of the healthy control, the connections within BLN of the patient subject are much more sparse, which may signal pathological changes in this neural system. For example, it is found that the patient has fewer connections between pyriform cortex (nodes 43, 44) and perirhinal cortex in the rhinal sulcus (nodes 55, 56) than healthy controls, and decreased connections between temporopolar area (nodes 61, 62) and retrosubicular area (nodes 81, 82).
These results are in line with previous studies \cite{das2020parietal, ferro2017longitudinal}. It finds that the parietal lobe, one of the major lobes in the brain roughly located at the upper back area in the skull and is in charge of processing sensory information received from the outside world, is mainly related to Bipolar disease attack. Since parietal lobe ROIs are contained in BLN under our parcellation, the connections missing within the BLN system in our visualization are consistent with existing clinical evidence.

\noindent \textbf{Interpretation of important brain systems.}
\begin{table}
% \setlength{\tabcolsep}{10pt}
	\centering
% 	\tiny
	\caption{Top ranked neural systems of the explanation subgraph on HIV and BP for both Healthy Control (Normal) and Patient under three comparative measures.}
	\resizebox{0.6\linewidth}{!}{
	\begin{tabular}{ccccc}
	\toprule
	\multirow{2.5}{*}{Dataset} & \multirow{2.5}{*}{Type} & \multicolumn{3}{c}{Comparative Measures} \\
	\cmidrule(lr){3-5}
	& & Degree & Strength & Cluster Coefficient  \\
	\midrule
	\multirow{2}{*}{HIV}
	& Normal   & DMN BLN CCN & DMN BLN CCN & DMN CCN BLN  \\
	& Patient  & BLN CCN AN & BLN CCN AN & BLN  \\
	\midrule
	\multirow{2}{*}{BP}
	& Normal & BLN SMN DMN & BLN DMN SMN & SMN VN DMN  \\
	& Patient & BLN DMN SMN & BLN DMN SMN & SMN VN \\
	\bottomrule
	\end{tabular}}
	
	\label{tab:metrics}
\end{table}
To understand which neural systems contribute most to the prediction of a specific disease, we observe the most manifest nodes on the explained subgraphs with three commonly used measures in brain network analysis: degree, strength, and cluster coefficient \cite{DBLP:journals/neuroimage/RubinovS10}. 
% The cluster coefficient of a node in a graph quantifies how close its neighbours are to being a clique (complete graph). Suppose the neighbourhood $\mathcal{N}_i$ for a node $v_i$ is its immediately connected neighbours $\mathcal{N}_{i}=\left\{v_{j}: e_{i j} \in \mathcal{E} \vee e_{j i} \in \mathcal{E}\right\}$ and $k_i$ is the number of neighbours of node $v_i$, the clustering coefficient for undirected graphs can be represented as 
% $$
% C_{i}=\frac{2\left|\left\{e_{j k}: v_{j}, v_{k} \in \mathcal{N}_{i}, e_{j k} \in \mathcal{E}\right\}\right|}{k_{i}\left(k_{i}-1\right)}.
% $$
As is shown in Table \ref{tab:metrics}, important neural systems under different metrics show similar characteristics. Specifically, for the HIV dataset, explanation subgraphs in both groups reveal the importance of BLN, while DMN is missing from all three metrics in the patient group. This is consistent with our observation on HIV in Figure \ref{fig:vis}, where the densely connected structure within DMN system degenerated in patient subjects. Regarding the BP dataset, BLN, SMN, and DMN are prominent in both patient and healthy controls. 

Furthermore, we compare the community structure and modularity  of our explanation graph $G^{\prime}$ against the original graph $G$ by conducting Newman's spectral community detection \cite{newman2013spectral}. The detected community results are compared with the ground truth neural system partition. Results show that the completeness score of our explained graph achieves about 7.21\% improvement over the original graph; the Fowlkes-Mallows score improves over 5.10\%; the homogeneity score improves 5.82\%; the mutual information score improves 5.12\% and the v-measure score improves over 6.44\%. The consistent improvements of various clustering evaluation metrics validate the effectiveness of our explanation mask: after applying the globally-shared explanation mask, the community characteristics are further manifest than the original graphs. 

\subsection{\hejie{Prediction Performance}}
We compare our proposed models with baselines from both shallow and deep models for performance evaluation. 

% \noindent \textbf{Metrics.}
% The metrics we used in experiments to evaluate performance are Accuracy and Area Under the ROC Curve (AUC), which are both widely used measures in healthcare domain. Larger values indicate better performance.

\noindent \textbf{Baselines.}
For shallow embeddings methods, we experimented M2E \cite{Liu:2018ty}, MIC \cite{Shao:2015ek}, MPCA \cite{Lu:2008cw}, and MK-SVM \cite{Dyrba:2015ci}, where the output graph-level embeddings are further processed by logistic regression classifiers to make predictions. We also include three state-of-the-art deep graph models: GAT \cite{Velickovic:2019tu}, GCN \cite{Kipf:2017tc}, and DiffPool \cite{Ying:2018vl}, \hejie{and two state-of-the-art deep models specifically design for brain networks: BrainnetCNN\cite{BrainNetCNN} and BrainGNN \cite{li2020braingnn}}.

\noindent \textbf{Results and analysis.}
\begin{table}
\setlength{\tabcolsep}{6pt}
	\centering
% 	\small
    % \scriptsize
	\caption{Performance of different models on \hejie{HIV, BP, and PPMI} datasets. Our proposed methods are colored in gray background and the highest performance is highlighted in boldface.}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{cccccccccc}
	\toprule
	\multirow{2.5}{*}{Method} & \multicolumn{3}{c}{HIV} & \multicolumn{3}{c}{BP} & \multicolumn{3}{c}{PPMI} \\
	\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
	& Accuracy & F1-macro & AUC & Accuracy & F1-macro & AUC & Accuracy & F1-macro & AUC \\
	\midrule
	M2E   & 57.14{\tiny±19.17} & 53.71{\tiny±19.80} & 57.50{\tiny±18.71} & 52.56{\tiny±13.86} & 51.65{\tiny±13.38} & 52.42{\tiny±13.83} & 78.69{\tiny±1.78} & 45.81{\tiny±4.17} & 50.39{\tiny±2.59}\\
	MIC   & 54.29{\tiny±18.95} & 53.63{\tiny±19.44} & 55.42{\tiny±19.10} & 62.67{\tiny±20.92} & 63.00{\tiny±21.61} & 61.79{\tiny±21.74} & 79.11{\tiny±2.16} & 49.65{\tiny±5.10} & 52.39{\tiny±2.94} \\
	MPCA  & 67.14{\tiny±20.25} & 64.28{\tiny±23.47} & 69.17{\tiny±20.17} & 52.56{\tiny±13.12} & 50.43{\tiny±14.99} & 52.42{\tiny±13.69} & 81.61{\tiny±2.64} & 62.45{\tiny±7.23} & 60.85{\tiny±5.48} \\
	MK-SVM & 65.71{\tiny±7.00} & 62.08{\tiny±7.49} & 65.83{\tiny±7.41} & 57.00{\tiny±8.89} & 41.08{\tiny±13.44} & 53.75{\tiny±8.00}     & 80.50{\tiny±2.73} & 67.98{\tiny±5.92} & 67.45{\tiny±6.30} \\
	\midrule
	GCN   & 70.00{\tiny±12.51} & 68.35{\tiny±13.28} & 73.58{\tiny±9.49} & 55.56{\tiny±13.86} & 50.71{\tiny±11.75} & 61.55{\tiny±28.77}  & 67.24{\tiny±5.51} & 67.24{\tiny±7.78} & 65.03{\tiny±6.23} \\
	GAT   & 71.43{\tiny±11.66} & 69.79{\tiny±10.83} & 77.17{\tiny±9.42} & 63.34{\tiny±9.15} &  60.42{\tiny±7.56} & 67.07{\tiny±5.98}    & 75.35{\tiny±2.23} & 64.04{\tiny±3.59} & 62.97{\tiny±3.06} \\
	PNA & 57.14{\tiny±12.78} & 45.09{\tiny±19.62} & 57.14{\tiny±12.78} & 63.71{\tiny±11.34} & 55.54{\tiny±14.06} & 60.30{\tiny±11.89}   & 80.36{\tiny±1.84} & 51.76{\tiny±10.32} & 54.71{\tiny±6.77}\\
	BrainCNN &  69.24{\tiny±19.04}& 67.08{\tiny±11.11} & 72.09{\tiny±19.01} & 65.83{\tiny±20.64} & 64.74{\tiny±17.42} & 64.32{\tiny±13.72} & 55.20{\tiny±12.63} & 55.45{\tiny±9.15} & 52.54{\tiny±10.21}\\
	BrainGNN & 74.29{\tiny±12.10} & 73.49{\tiny±10.75} & 75.00{\tiny±10.56} & 68.00{\tiny±12.45} & 62.33{\tiny±13.01} & 74.20{\tiny±12.93} &69.17{\tiny±0.00}  & 44.19{\tiny±0.00} &45.26{\tiny±3.65}\\
	\midrule 
	\rowcolor{lightgray!20} \back & 82.14{\tiny±10.81} & 82.02{\tiny±10.86} & 86.86{\tiny±11.65} & 73.19{\tiny±12.20} & 72.87{\tiny±12.09} & 83.64{\tiny±9.61} & 78.78{\tiny±1.44} & 44.06{\tiny±0.46} & 52.51{\tiny±5.92} \\
	\rowcolor{lightgray!20} \ours & \textbf{84.29}{\tiny±12.94} & \textbf{83.86}{\tiny±13.42} & \textbf{88.57}{\tiny±10.89} & \textbf{76.33}{\tiny±13.00} & 76.13{\tiny±13.01} & \textbf{84.61}{\tiny±9.08} & 75.60{\tiny±3.49} & 60.63{\tiny±6.67} & 54.72{\tiny±6.51} \\
	\bottomrule
	\end{tabular}}
	\label{tab:performance}
\end{table}
The overall results are presented in Table \ref{tab:performance}, where our proposed methods are colored gray. Impressively, both \back and \ours yield significant and consistent improvements over all SOTA shallow and deep baselines. Compared with traditional shallow models such as MK-SVM, our backbone \back outperforms them by large margins, with up to 11\% absolute improvements on BP, which demonstrates the potential of using deep GNNs on brain networks. The rationale of our edge-weight-aware message passing is supported by the superiority of \back compared with other SOTA deep models such as GAT. Based on this backbone, the performance of \ours achieves a further increase of about 5\% absolute improvements \hejie{by tuning the parameters on the enhanced graphs}. The gain comes from the explanation generator, which addresses the problem of edge weight noises \hejie{and highlight the disease-specific signals} contained in the original graph through a \hejie{across-instance} mask.
This outstanding performance of \ours certifies the disease-specific interpretability of our explanation mask and effectiveness of the proposed \hejie{end-to-end} framework. 

==> trash/method.tex <==
\section{Methods}


\subsection{Problem Setting}

\noindent \textbf{Problem Setup and Notations.}
Given a weighted brain network \(G = (\mathcal{V}, \mathcal{E}, \bm{W})\), where \(\mathcal{V} = \{v_i\}_{i = 1}^m\) is the node set of size \(m\) defined by the regions of interest (ROIs) \hejie{on a specific brain parcellation \cite{figley2017probabilistic, shirer2012decoding}}, \(\mathcal{E} = \mathcal{V} \times \mathcal{V}\) is the edge set, and \(\bm{W} \in \mathbb{R}^{m \times m}\) is the weighted adjacency matrix describing connection strengths between ROIs, the model outputs a disease prediction \(\hat{y}\). The interpretability is provided by learning an edge mask \(\bm{M} \in \mathbb{R}^{m\times m}\) shared across all subjects to highlight the disease-specific prominent ROI connections. 

\noindent \textbf{Class Incremental Learning}

\noindent \textbf{Dream Data}

\noindent \textbf{Research Challenges to be solved}

Here we propose a complete novel 


\subsection{Our Proposed Methods}
\label{sec:overall}
% \noindent \textbf{Three-step training strategy.}
Overall, \ours is trained \hejie{end-to-end iteratively} as shown in Figure \ref{fig:framework}. In particular, a backbone \back model is first trained on the original data, as described in Section \ref{sec:predict}. Using this trained model and its prediction as the input, the explanation generator then learns \hejie{a shared explanation mask across all training instances}. Finally, we apply the learned global mask $\bm M$ on the original training graph $G$ to get an \hejie{explanation enhanced graph $G^{\prime}$, then use it to tune  parameters in \back again. With this iterative process, we further improve the prediction performance and at the same time obtain a novel across-instance explanation mask for brain analysis}.

